Determinization of Min-Plus Weighted Automata is Decidable

We show that the determinization problem for min-plus (tropical) weighted automata is decidable, thus resolving this long-standing open problem. In doing so, we develop a new toolbox for analyzing and reasoning about the run-structure of nondeterministic automata.

==> fig/IncreasingInfix.tex <==
\begin{tikzpicture}[scale=1.5, every node/.style={draw, circle, inner sep=1pt}]

% Root node
\node (root) at (-2.5, -2) {$p$};

% Bottom segment labels with segment width representation
\draw[thick] (-2.5, -3.9) -- (-0.5, -3.9) node[midway, below, draw=none] {$u$};
\draw[thick] (-2.5, -3.9) -- ++(0, 0.2);
\draw[thick] (-0.5, -3.9) -- ++(0, 0.2);

\draw[thick] (-0.5, -3.9) -- (0.5, -3.9) node[midway, below, draw=none] {$x$};
\draw[thick] (-0.5, -3.9) -- ++(0, 0.2);
\draw[thick] (0.5, -3.9) -- ++(0, 0.2);

\draw[thick] (0.5, -3.9) -- (3, -3.9) node[midway, below, draw=none] {$y$};
\draw[thick] (0.5, -3.9) -- ++(0, 0.2);
\draw[thick] (3, -3.9) -- ++(0, 0.2);

\draw[thick] (3, -3.9) -- (4, -3.9) node[midway, below, draw=none] {$z$};
\draw[thick] (3, -3.9) -- ++(0, 0.2);
\draw[thick] (4, -3.9) -- ++(0, 0.2);




% First set of vertical nodes after u
\node (u1a) at (-0.5, -3.5) {};
\node (u1b) at (-0.5, -3.35) {};

\node (u2a) at (-0.5, -2.5) {};
\node (u2b) at (-0.5, -2.35) {};
\node (u2c) at (-0.5, -2.2) {};

\node (u3a) at (-0.5, -1.2) {};
\node (u3b) at (-0.5, -1.05) {};

% Semi-transparent frame around the first set
\begin{pgfonlayer}{background}
\fill[red!30, rounded corners] (-0.7, -3.7) rectangle (-0.3, -3.15);
\end{pgfonlayer}
\begin{pgfonlayer}{background}
\fill[green!30, rounded corners] (-0.7, -2.7) rectangle (-0.3, -2);
\end{pgfonlayer}
\begin{pgfonlayer}{background}
\fill[yellow!30, rounded corners] (-0.7, -1.4) rectangle (-0.3, -0.85);
\end{pgfonlayer}

% Second set of vertical nodes after x
\pgfmathsetmacro{\offoneone}{0.1}
\pgfmathsetmacro{\offonetwo}{0.5}
\pgfmathsetmacro{\offonethree}{0.3}
\node (x1a) at ($(0.5, -3.5) + (0,\offoneone)$) {};
\node (x1b) at ($(0.5, -3.35) + (0,\offoneone)$) {};

\node (x2a) at ($(0.5, -2.5) + (0,\offonetwo)$) {};
\node (x2b) at ($(0.5, -2.35) + (0,\offonetwo)$) {};
\node (x2c) at ($(0.5, -2.2) + (0,\offonetwo)$) {};

\node (x3a) at ($(0.5, -1.2) + (0,\offonethree)$) {};
\node (x3b) at ($(0.5, -1.05) + (0,\offonethree)$) {};
% Semi-transparent frame around the second set
\begin{pgfonlayer}{background}
\fill[red!30, rounded corners] ($(0.3, -3.7) + (0,\offoneone)$) rectangle ($(0.7, -3.15)+ (0,\offoneone)$);
\end{pgfonlayer}
% Double sided arrow with "gap" label
\draw[<->, blue!50] ($(0.5, -3.15) + (0,\offoneone)$) -- node[midway, draw=none, fill=white,minimum size=0pt, inner sep=0pt] {\small gap} ($(0.5, -2.7) + (0,\offonetwo)$);
\begin{pgfonlayer}{background}
\fill[green!30, rounded corners] ($(0.3, -2.7)+ (0,\offonetwo)$) rectangle ($(0.7, -2)+ (0,\offonetwo)$);
\end{pgfonlayer}
\begin{pgfonlayer}{background}
\fill[yellow!30, rounded corners] ($(0.3, -1.4)+ (0,\offonethree)$) rectangle ($(0.7, -0.85)+ (0,\offonethree)$);
\end{pgfonlayer}

% Third set of vertical nodes after y
\pgfmathsetmacro{\offtwoone}{0.7}
\pgfmathsetmacro{\offtwotwo}{0.7}
\pgfmathsetmacro{\offtwothree}{0.4}
\node (y1a) at ($(3, -3.5) + (0,\offtwoone)$) {};
\node (y1b) at ($(3, -3.35) + (0,\offtwoone)$) {};
\node (y2a) at ($(3, -2.5) + (0,\offtwotwo)$) {};
\node (y2b) at ($(3, -2.35) + (0,\offtwotwo)$) {};
\node (y2c) at ($(3, -2.2) + (0,\offtwotwo)$) {};
\node (y3a) at ($(3, -1.2) + (0,\offtwothree)$) {};
\node (y3b) at ($(3, -1.05) + (0,\offtwothree)$) {};

% Semi-transparent frame around the third set
\begin{pgfonlayer}{background}
    \fill[red!30, rounded corners] ($(2.8, -3.7) + (0,\offtwoone)$) rectangle ($(3.2, -3.15)+ (0,\offtwoone)$);
    \end{pgfonlayer}
    \begin{pgfonlayer}{background}
    \fill[green!30, rounded corners] ($(2.8, -2.7)+ (0,\offtwotwo)$) rectangle ($(3.2, -2)+ (0,\offtwotwo)$);
    \end{pgfonlayer}
    \begin{pgfonlayer}{background}
    \fill[yellow!30, rounded corners] ($(2.8, -1.4)+ (0,\offtwothree)$) rectangle ($(3.2, -0.85)+ (0,\offtwothree)$);
    \end{pgfonlayer}

% Fourth set of vertical nodes after z
\node (z1a) at (4, -3.5) {};
\node (z1b) at (4, -3.0) {};
\node (z2a) at (4, -2.5) {};
\node (z2b) at (4, -2.0) {};
\node (z2c) at (4, -1.5) {};
\node (z3a) at (4, -1.0) {};
\node (z3b) at (4, -0.5) {};

% Semi-transparent frame around the fourth set
% \begin{pgfonlayer}{background}
% \fill[blue!30, rounded corners] (3.8, -3.7) rectangle (4.2, 0.2);
% \end{pgfonlayer}

% Invisible nodes for tree-like structure
\node (mid1) at (-1.9, -2.3) [draw=none, minimum size=1pt, inner sep=0pt] {};
\node (mid2) at (-1.4, -1.8) [draw=none, minimum size=0pt, inner sep=0pt] {};
\node (mid3) at (-1.7, -1.4) [draw=none, minimum size=0pt, inner sep=0pt] {};

% Connections from root to first set (tree-like structure)
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid1) -- (u1a);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid2) -- (u1b);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid3) -- (u2a);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid1) -- (u2b);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid2) -- (u2c);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid3) -- (u3a);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (root) -- (mid1) -- (u3b);

% % Additional branches for tree-like structure
% \draw[decorate, decoration={snake, amplitude=0.5mm, segment length=4mm}] (root) to[out=210, in=160] (u1a);
% \draw[decorate, decoration={snake, amplitude=0.5mm, segment length=4mm}] (root) to[out=250, in=200] (u1b);

% Connections between sets (u -> x)
\node[draw=none] at ($(u1a)!0.5!(x1a)+(0,0.35)$) {\small $+k_{1,x}$};
\draw (u1a) -- (x1a);
\draw (u1b) -- (x1b);

\node[draw=none] at ($(u2a)!0.5!(x2a)+(0,0.55)$) {\small $+k_{2,x}$};
\draw (u2a) -- (x2a);
\draw (u2b) -- (x2b);
\draw (u2c) -- (x2c);

\node[draw=none] at ($(u3a)!0.5!(x3a)+(0,0.4)$) {\small $+k_{3,x}$};
\draw (u3a) -- (x3a);
\draw (u3b) -- (x3b);

% Connections between sets (x -> y)
\node[draw=none] at ($(x1a)!0.5!(y1a)+(0,0.35)$) {\small $+k_{1,y}$};
\node[draw=none] at ($(x2a)!0.5!(y2a)+(0,0.5)$) {\small $+k_{2,y}$};
\node[draw=none] at ($(x3a)!0.5!(y3a)+(0,0.35)$) {\small $+k_{3,y}$};
\draw (x1a) -- (y1a);
\draw (x1b) -- (y1b);
\draw (x2a) -- (y2a);
\draw (x2b) -- (y2b);
\draw (x2c) -- (y2c);
\draw (x3a) -- (y3a);
\draw (x3b) -- (y3b);

% Connections between sets (y -> z)
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y1a) -- (z1a);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y1b) -- (z1b);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y2a) -- (z2a);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y2b) -- (z2b);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y2c) -- (z2c);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y3a) -- (z3a);
\draw[gray, decorate, decoration={snake, amplitude=0.3mm, segment length=4mm}] (y3b) -- (z3b);

\end{tikzpicture}
